Demystify Adult Learning: A Social Network and Large Language Model Assisted Approach

Adult learning is increasingly recognized as a crucial way for personal development and societal progress. It however is challenging, and adult learners face unique challenges such as balancing education with other life responsibilities. Collecting feedback from adult learners is effective in understanding their concerns and improving learning experiences, and social networks provide a rich source of real-time sentiment data from adult learners. Machine learning technologies especially large language models (LLMs) perform well in automating sentiment analysis. However, none of such models is specialized for adult learning with accurate sentiment understanding. In this paper, we present A-Learn, which enhances adult learning sentiment analysis by customizing existing general-purpose LLMs with domain-specific datasets for adult learning. We collect adult learners' comments from social networks and label the sentiment of each comment with an existing LLM to form labelled datasets tailored for adult learning. The datasets are used to customize A-Learn from several base LLMs. We conducted experimental studies and the results reveal A-Learn's competitive sentiment analysis performance, achieving up to 91.3% accuracy with 20% improvement over the base LLM. A-Learn is also employed for word cloud analysis to identify key concerns of adult learners. The research outcome of this study highlights the importance of applying machine learning with educational expertise for teaching improvement and educational innovations that benefit adult learning and adult learners.

==> tmp.tex <==
@article{
Liang-MisinformationSocialMedia,
author = {Wu, Liang and Morstatter, Fred and Carley, Kathleen M. and Liu, Huan},
title = {Misinformation in Social Media: Definition, Manipulation, and Detection},
year = {2019},
issue_date = {December 2019},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
volume = {21},
number = {2},
issn = {1931-0145},
doi = {10.1145/3373464.3373475},
journal = {SIGKDD Explor. Newsl.},
month = {nov},
pages = {80–90},
numpages = {11}
}

@ARTICLE{
Gabarron2021-bw,
  title    = "{COVID-19-related} misinformation on social media: a systematic review",
  author   = "Gabarron, Elia and Oyeyemi, Sunday Oluwafemi and Wynn, Rolf",
  journal  = "Bull World Health Organ",
  volume   =  99,
  number   =  6,
  pages    = "455--463A",
  month    =  mar,
  year     =  2021,
  address  = "Switzerland",
  language = "en"
}

@ARTICLE{
Joseph2022-ro,
  title    = "{COVID-19} Misinformation on Social Media: A Scoping Review",
  author   = "Joseph, Andrew M and Fernandez, Virginia and Kritzman, Sophia and Eaddy, Isabel and Cook, Olivia M and Lambros, Sarah and Jara Silva, Cesar E and Arguelles, Daryl and Abraham, Christy and Dorgham, Noelle and Gilbert, Zachary A and Chacko, Lindsey and Hirpara, Ram J and Mayi, Bindu S and Jacobs, Robin J",
  journal  = "Cureus",
  volume   =  14,
  number   =  4,
  pages    = "e24601",
  month    =  apr,
  year     =  2022,
  address  = "United States",
  keywords = "coronavirus; covid-19; disinformation; facebook; misinformation; pandemic; sars-cov-2; social media; twitter; youtube",
  language = "en"
}

@ARTICLE{Muhammed_T2022-ra,
  title    = "The disaster of misinformation: a review of research in social
              media",
  author   = "Muhammed T, Sadiq and Mathew, Saji K",
  journal  = "Int J Data Sci Anal",
  volume   =  13,
  number   =  4,
  pages    = "271--285",
  month    =  feb,
  year     =  2022,
  address  = "Switzerland",
  keywords = "Information disorder; Misinformation; Social media; Systematic
              literature review",
  language = "en"
}

@Article{
Wani-impactUnreliableContent,
AUTHOR = {Wani, Mudasir Ahmad and Agarwal, Nancy and Bours, Patrick},
TITLE = {Impact of Unreliable Content on Social Media Users during COVID-19 and Stance Detection System},
JOURNAL = {Electronics},
VOLUME = {10},
YEAR = {2021},
NUMBER = {1},
ARTICLE-NUMBER = {5},
ISSN = {2079-9292},
DOI = {10.3390/electronics10010005}
}


@Article{Jennings-SocialMediaVaccine,
AUTHOR = {Jennings, Will and Stoker, Gerry and Bunting, Hannah and Valgarðsson, Viktor Orri and Gaskell, Jennifer and Devine, Daniel and McKay, Lawrence and Mills, Melinda C.},
TITLE = {Lack of Trust, Conspiracy Beliefs, and Social Media Use Predict COVID-19 Vaccine Hesitancy},
JOURNAL = {Vaccines},
VOLUME = {9},
YEAR = {2021},
NUMBER = {6},
ARTICLE-NUMBER = {593},
PubMedID = {34204971},
ISSN = {2076-393X},
DOI = {10.3390/vaccines9060593}
}

@ARTICLE{Roozenbeek2020-og,
  title    = "Susceptibility to misinformation about {COVID-19} around the
              world",
  author   = "Roozenbeek, Jon and Schneider, Claudia R and Dryhurst, Sarah and
              Kerr, John and Freeman, Alexandra L J and Recchia, Gabriel and
              van der Bles, Anne Marthe and van der Linden, Sander",
  journal  = "R Soc Open Sci",
  volume   =  7,
  number   =  10,
  pages    = "201199",
  month    =  oct,
  year     =  2020,
  address  = "England",
  keywords = "COVID-19; fake news; misinformation; vaccine hesitancy",
  language = "en"
}

@ARTICLE{Chen2022-ib,
  title    = "Infodemic, Institutional Trust, and {COVID-19} Vaccine Hesitancy:
              A {Cross-National} Survey",
  author   = "Chen, Xi and Lee, Woohyung and Lin, Fen",
  journal  = "Int J Environ Res Public Health",
  volume   =  19,
  number   =  13,
  month    =  jun,
  year     =  2022,
  address  = "Switzerland",
  keywords = "COVID-19; infodemic; information overload; institutional trust;
              misinformation; vaccine hesitancy",
  language = "en"
}

@ARTICLE{Ahmed2022-tf,
  title    = "Social Media News Use and {COVID-19} Misinformation Engagement:
              Survey Study",
  author   = "Ahmed, Saifuddin and Rasul, Muhammad Ehab",
  journal  = "J Med Internet Res",
  volume   =  24,
  number   =  9,
  pages    = "e38944",
  month    =  sep,
  year     =  2022,
  address  = "Canada",
  keywords = "COVID-19; Singapore; cognitive ability; misinformation;
              personality; social media",
  language = "en"
}

@article{Al-Zaman-ignorantFacebook,
title = {Social media and COVID-19 misinformation: how ignorant Facebook users are?},
journal = {Heliyon},
volume = {7},
number = {5},
pages = {e07144},
year = {2021},
issn = {2405-8440},
doi = {https://doi.org/10.1016/j.heliyon.2021.e07144},
author = {Md. Sayeed Al-Zaman},
keywords = {Social media, Ignorance, Misinformation, COVID-19, Facebook},
}

@misc{brennen2020a,
  edition = {},
  number = {},
  journal = {},
  pages = {},
  publisher = {Reuters Institute for the Study of Journalism},
  school = {University of Oxford},
  title = {Types, sources, and claims of COVID-19 misinformation},
  volume = {},
  author = {Brennen, JS and Simon, FM and Howard, PN and Nielsen, RK},
  editor = {},
  year = {2020},
  series = {}
}

@INPROCEEDINGS{Kumar-fakeNewsMLReview,
  author={Kumar, Sunil and Arora, Bhavna},
  booktitle={2021 Second International Conference on Electronics and Sustainable Communication Systems (ICESC)}, 
  title={A Review of Fake News Detection Using Machine Learning Techniques}, 
  year={2021},
  volume={},
  number={},
  pages={1-8},
  doi={10.1109/ICESC51422.2021.9532796}}

@ARTICLE{Shah-fakeNewsMLReview,
  title    = "A systematic literature review and existing challenges toward
              fake news detection models",
  author   = "Nirav Shah, Minal and Ganatra, Amit",
  journal  = "Social Network Analysis and Mining",
  volume   =  12,
  number   =  1,
  pages    = "168",
  month    =  nov,
  year     =  2022
}

@article{Hu-fakeNewsMLReview,
title = {Deep learning for fake news detection: A comprehensive survey},
journal = {AI Open},
volume = {3},
pages = {133-155},
year = {2022},
issn = {2666-6510},
doi = {j.aiopen.2022.09.001},
author = {Linmei Hu and Siqi Wei and Ziwang Zhao and Bin Wu},
keywords = {Fake news detection, Deep learning},
}

@InProceedings{
    parth2021Infodemic,
    author="Patwa, Parth
    and Sharma, Shivam
    and Pykl, Srinivas
    and Guptha, Vineeth
    and Kumari, Gitanjali
    and Akhtar, Md Shad
    and Ekbal, Asif
    and Das, Amitava
    and Chakraborty, Tanmoy",
    editor="Chakraborty, Tanmoy
    and Shu, Kai
    and Bernard, H. Russell
    and Liu, Huan
    and Akhtar, Md Shad",
    title="Fighting an Infodemic: COVID-19 Fake News Dataset",
    booktitle="Combating Online Hostile Posts in Regional Languages during Emergency Situation",
    year="2021",
    publisher="Springer International Publishing",
    address="Cham",
    pages="21--29",
    isbn="978-3-030-73696-5"
}

@article{Tausczik-LIWC,
author = {Yla R. Tausczik and James W. Pennebaker},
title ={The Psychological Meaning of Words: LIWC and Computerized Text Analysis Methods},
journal = {Journal of Language and Social Psychology},
volume = {29},
number = {1},
pages = {24-54},
year = {2010},
doi = {10.1177/0261927X09351676},
}

@ARTICLE{Hearst-SVM,
  author={Hearst, M.A. and Dumais, S.T. and Osuna, E. and Platt, J. and Scholkopf, B.},
  journal={IEEE Intelligent Systems and their Applications}, 
  title={Support vector machines}, 
  year={1998},
  volume={13},
  number={4},
  pages={18-28},
  doi={10.1109/5254.708428}}

@ARTICLE{Breiman2001-ib,
  title    = "Random Forests",
  author   = "Breiman, Leo",
  journal  = "Machine Learning",
  volume   =  45,
  number   =  1,
  pages    = "5--32",
  month    =  oct,
  year     =  2001
}

@inproceedings{Tianqi-xgboost,
author = {Chen, Tianqi and Guestrin, Carlos},
title = {XGBoost: A Scalable Tree Boosting System},
year = {2016},
isbn = {9781450342322},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
doi = {10.1145/2939672.2939785},
booktitle = {Proceedings of the 22nd ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
pages = {785–794},
numpages = {10},
keywords = {large-scale machine learning},
location = {San Francisco, California, USA},
series = {KDD '16}
}

@article{hendrycks2016gelu,
  title={Gaussian Error Linear Units (GELUs)},
  author={Hendrycks, Dan and Gimpel, Kevin},
  journal={arXiv preprint arXiv:1606.08415},
  year={2016}
}

@article{srivastava-dropout,
  author  = {Nitish Srivastava and Geoffrey Hinton and Alex Krizhevsky and Ilya Sutskever and Ruslan Salakhutdinov},
  title   = {Dropout: A Simple Way to Prevent Neural Networks from Overfitting},
  journal = {Journal of Machine Learning Research},
  year    = {2014},
  volume  = {15},
  number  = {56},
  pages   = {1929--1958},
}

@inproceedings{
loshchilov2018decoupled,
title={Decoupled Weight Decay Regularization},
author={Ilya Loshchilov and Frank Hutter},
booktitle={International Conference on Learning Representations},
year={2019},
}

@InProceedings{KingBa15,
  author    = {Kingma, Diederik and Ba, Jimmy},
  booktitle = {International Conference on Learning Representations (ICLR)},
  title     = {Adam: A Method for Stochastic Optimization},
  year      = {2015},
  address   = {San Diega, CA, USA},
  optmonth  = {12},
}

@inproceedings{
Lan2020ALBERT,
title={ALBERT: A Lite BERT for Self-supervised Learning of Language Representations},
author={Zhenzhong Lan and Mingda Chen and Sebastian Goodman and Kevin Gimpel and Piyush Sharma and Radu Soricut},
booktitle={International Conference on Learning Representations},
year={2020},
}

@inproceedings{devlin-etal-2019-bert,
    title = "{BERT}: Pre-training of Deep Bidirectional Transformers for Language Understanding",
    author = "Devlin, Jacob  and
      Chang, Ming-Wei  and
      Lee, Kenton  and
      Toutanova, Kristina",
    booktitle = "Proceedings of the 2019 Conference of the North {A}merican Chapter of the Association for Computational Linguistics: Human Language Technologies, Volume 1 (Long and Short Papers)",
    month = jun,
    year = "2019",
    address = "Minneapolis, Minnesota",
    publisher = "Association for Computational Linguistics",
    doi = "10.18653/v1/N19-1423",
    pages = "4171--4186",
}

@inproceedings{nguyen-etal-2020-bertweet,
    title = "{BERT}weet: A pre-trained language model for {E}nglish Tweets",
    author = "Nguyen, Dat Quoc  and
      Vu, Thanh  and
      Tuan Nguyen, Anh",
    booktitle = "Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing: System Demonstrations",
    month = oct,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    doi = "10.18653/v1/2020.emnlp-demos.2",
    pages = "9--14",
}

@ARTICLE{Muller2023-ke,
  title    = "{COVID-Twitter-BERT}: A natural language processing model to
              analyse {COVID-19} content on Twitter",
  author   = "M{\"u}ller, Martin and Salath{\'e}, Marcel and Kummervold, Per E",
  journal  = "Front Artif Intell",
  volume   =  6,
  pages    = "1023281",
  month    =  mar,
  year     =  2023,
  address  = "Switzerland",
  keywords = "BERT; COVID-19; language model (LM); natural language processing
              (NLP); text classification",
  language = "en"
}

@article{victor-distilbert,
  author       = {Victor Sanh and
                  Lysandre Debut and
                  Julien Chaumond and
                  Thomas Wolf},
  title        = {DistilBERT, a distilled version of {BERT:} smaller, faster, cheaper
                  and lighter},
  journal      = {CoRR},
  volume       = {abs/1910.01108},
  year         = {2019},
  url          = {http://arxiv.org/abs/1910.01108},
  eprinttype    = {arXiv},
  eprint       = {1910.01108},
  timestamp    = {Tue, 02 Jun 2020 12:48:59 +0200},
  biburl       = {https://dblp.org/rec/journals/corr/abs-1910-01108.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@misc{beltagy2020longformer,
      title={Longformer: The Long-Document Transformer}, 
      author={Iz Beltagy and Matthew E. Peters and Arman Cohan},
      year={2020},
      eprint={2004.05150},
      archivePrefix={arXiv},
      primaryClass={cs.CL}
}

@misc{
liu2020roberta,
title={Ro{\{}BERT{\}}a: A Robustly Optimized {\{}BERT{\}} Pretraining Approach},
author={Yinhan Liu and Myle Ott and Naman Goyal and Jingfei Du and Mandar Joshi and Danqi Chen and Omer Levy and Mike Lewis and Luke Zettlemoyer and Veselin Stoyanov},
year={2020},
}

@inproceedings{barbieri-etal-2020-tweeteval,
    title = "{T}weet{E}val: Unified Benchmark and Comparative Evaluation for Tweet Classification",
    author = "Barbieri, Francesco  and
      Camacho-Collados, Jose  and
      Espinosa Anke, Luis  and
      Neves, Leonardo",
    booktitle = "Findings of the Association for Computational Linguistics: EMNLP 2020",
    month = nov,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.findings-emnlp.148",
    doi = "10.18653/v1/2020.findings-emnlp.148",
    pages = "1644--1650",
}

@inproceedings{Conneau-xlm,
 author = {Conneau, Alexis and Lample, Guillaume},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {Cross-lingual Language Model Pretraining},
 url = {https://proceedings.neurips.cc/paper_files/paper/2019/file/c04c19c2c2474dbf5f7ac4372c5b9af1-Paper.pdf},
 volume = {32},
 year = {2019}
}


@inproceedings{
    Conneau-xlm-r,
    title = "Unsupervised Cross-lingual Representation Learning at Scale",
    author = "Conneau, Alexis  and
      Khandelwal, Kartikay  and
      Goyal, Naman  and
      Chaudhary, Vishrav  and
      Wenzek, Guillaume  and
      Guzm{\'a}n, Francisco  and
      Grave, Edouard  and
      Ott, Myle  and
      Zettlemoyer, Luke  and
      Stoyanov, Veselin",
    booktitle = "Proceedings of the 58th Annual Meeting of the Association for Computational Linguistics",
    month = jul,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.acl-main.747",
    doi = "10.18653/v1/2020.acl-main.747",
    pages = "8440--8451",
}

@inproceedings{Zhilin-xlnet,
 author = {Yang, Zhilin and Dai, Zihang and Yang, Yiming and Carbonell, Jaime and Salakhutdinov, Russ R and Le, Quoc V},
 booktitle = {Advances in Neural Information Processing Systems},
 editor = {H. Wallach and H. Larochelle and A. Beygelzimer and F. d\textquotesingle Alch\'{e}-Buc and E. Fox and R. Garnett},
 pages = {},
 publisher = {Curran Associates, Inc.},
 title = {XLNet: Generalized Autoregressive Pretraining for Language Understanding},
 url = {https://proceedings.neurips.cc/paper_files/paper/2019/file/dc6a7e655d7e5840e66733e9ee67cc69-Paper.pdf},
 volume = {32},
 year = {2019}
}

@misc{cui2020coaid,
    title={CoAID: COVID-19 Healthcare Misinformation Dataset},
    author={Limeng Cui and Dongwon Lee},
    year={2020},
    eprint={2006.00885},
    archivePrefix={arXiv},
    primaryClass={cs.SI}
}

@inproceedings{Zhou-recovery,
author = {Zhou, Xinyi and Mulay, Apurva and Ferrara, Emilio and Zafarani, Reza},
title = {ReCOVery: A Multimodal Repository for COVID-19 News Credibility Research},
year = {2020},
isbn = {9781450368599},
publisher = {Association for Computing Machinery},
address = {New York, NY, USA},
url = {https://doi.org/10.1145/3340531.3412880},
doi = {10.1145/3340531.3412880},
booktitle = {Proceedings of the 29th ACM International Conference on Information \& Knowledge Management},
pages = {3205–3212},
numpages = {8},
keywords = {covid-19, information credibility, infodemic, social media, pandemic, multimodal, repository, coronavirus, fake news},
location = {Virtual Event, Ireland},
series = {CIKM '20}
}

@inproceedings{shahifakecovid,
title={Fake{C}ovid -- A Multilingual Cross-domain Fact Check News Dataset for COVID-19},
author={Shahi, Gautam Kishore and Nandini, Durgesh},
booktitle={Workshop Proceedings of the 14th International {AAAI} {C}onference on {W}eb and {S}ocial {M}edia},
year = {2020},
url = {http://workshop-proceedings.icwsm.org/pdf/2020_14.pdf}
}

@ARTICLE{Shuja2020-tc,
  title    = "{COVID-19} open source data sets: a comprehensive survey",
  author   = "Shuja, Junaid and Alanazi, Eisa and Alasmary, Waleed and
              Alashaikh, Abdulaziz",
  journal  = "Appl Intell (Dordr)",
  volume   =  51,
  number   =  3,
  pages    = "1296--1325",
  month    =  sep,
  year     =  2020,
  address  = "Netherlands",
  keywords = "Artificial intelligence; COVID-19; Coronavirus; Data sets;
              Machine learning; Open source; Pandemic",
  language = "en"
}

@ARTICLE{Latif-leveragingDS,
  author={Latif, Siddique and Usman, Muhammad and Manzoor, Sanaullah and Iqbal, Waleed and Qadir, Junaid and Tyson, Gareth and Castro, Ignacio and Razi, Adeel and Boulos, Maged N. Kamel and Weller, Adrian and Crowcroft, Jon},
  journal={IEEE Transactions on Artificial Intelligence}, 
  title={Leveraging Data Science to Combat COVID-19: A Comprehensive Review}, 
  year={2020},
  volume={1},
  number={1},
  pages={85-103},
  doi={10.1109/TAI.2020.3020521}}

@ARTICLE{Hayawi2021-qs,
  title    = "{ANTi-Vax}: a novel Twitter dataset for {COVID-19} vaccine
              misinformation detection",
  author   = "Hayawi, K and Shahriar, S and Serhani, M A and Taleb, I and
              Mathew, S S",
  journal  = "Public Health",
  volume   =  203,
  pages    = "23--30",
  month    =  dec,
  year     =  2021,
  address  = "Netherlands",
  keywords = "COVID-19; Deep learning; Misinformation detection; Natural
              language processing; Text classification; Vaccines",
  language = "en"
}

@ARTICLE{cheema-fakenews,
       author = {{Cheema}, Gullal S. and {Hakimov}, Sherzod and {Ewerth}, Ralph},
        title = "{TIB's Visual Analytics Group at MediaEval '20: Detecting Fake News on Corona Virus and 5G Conspiracy}",
      journal = {arXiv e-prints},
     keywords = {Computer Science - Social and Information Networks, Computer Science - Computation and Language},
         year = 2021,
        month = jan,
          eid = {arXiv:2101.03529},
        pages = {arXiv:2101.03529},
          doi = {10.48550/arXiv.2101.03529},
archivePrefix = {arXiv},
       eprint = {2101.03529},
 primaryClass = {cs.SI},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210103529C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{Hande-fakenews,
  author={Hande, Adeep and Puranik, Karthik and Priyadharshini, Ruba and Thavareesan, Sajeetha and Chakravarthi, Bharathi Raja},
  booktitle={2021 5th International Conference on Computing Methodologies and Communication (ICCMC)}, 
  title={Evaluating Pretrained Transformer-based Models for COVID-19 Fake News Detection}, 
  year={2021},
  volume={},
  number={},
  pages={766-772},
  doi={10.1109/ICCMC51019.2021.9418446}}

@inproceedings{hossain-etal-2020-covidlies,
    title = "{COVIDL}ies: Detecting {COVID}-19 Misinformation on Social Media",
    author = "Hossain, Tamanna  and
      Logan IV, Robert L.  and
      Ugarte, Arjuna  and
      Matsubara, Yoshitomo  and
      Young, Sean  and
      Singh, Sameer",
    booktitle = "Proceedings of the 1st Workshop on {NLP} for {COVID}-19 (Part 2) at {EMNLP} 2020",
    month = dec,
    year = "2020",
    address = "Online",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/2020.nlpcovid19-2.11",
    doi = "10.18653/v1/2020.nlpcovid19-2.11",
}

@inproceedings{bert-score,
  title={BERTScore: Evaluating Text Generation with BERT},
  author={Tianyi Zhang* and Varsha Kishore* and Felix Wu* and Kilian Q. Weinberger and Yoav Artzi},
  booktitle={International Conference on Learning Representations},
  year={2020},
  url={https://openreview.net/forum?id=SkeHuCVFDr}
}

@inproceedings{pennington-etal-2014-glove,
    title = "{G}lo{V}e: Global Vectors for Word Representation",
    author = "Pennington, Jeffrey  and
      Socher, Richard  and
      Manning, Christopher",
    booktitle = "Proceedings of the 2014 Conference on Empirical Methods in Natural Language Processing ({EMNLP})",
    month = oct,
    year = "2014",
    address = "Doha, Qatar",
    publisher = "Association for Computational Linguistics",
    url = "https://aclanthology.org/D14-1162",
    doi = "10.3115/v1/D14-1162",
    pages = "1532--1543",
}

@INPROCEEDINGS{pavlov-fakenews,
  author={Pavlov, Tashko and Mirceva, Georgina},
  booktitle={2022 45th Jubilee International Convention on Information, Communication and Electronic Technology (MIPRO)}, 
  title={COVID-19 Fake News Detection by Using BERT and RoBERTa models}, 
  year={2022},
  volume={},
  number={},
  pages={312-316},
  doi={10.23919/MIPRO55190.2022.9803414}}

@article{Gundapu-transformerEnsemble,
  author       = {Sunil Gundapu and
                  Radhika Mamidi},
  title        = {Transformer based Automatic {COVID-19} Fake News Detection System},
  journal      = {CoRR},
  volume       = {abs/2101.00180},
  year         = {2021},
  url          = {https://arxiv.org/abs/2101.00180},
  eprinttype    = {arXiv},
  eprint       = {2101.00180},
  timestamp    = {Thu, 21 Jan 2021 14:42:30 +0100},
  biburl       = {https://dblp.org/rec/journals/corr/abs-2101-00180.bib},
  bibsource    = {dblp computer science bibliography, https://dblp.org}
}

@InProceedings{Glazkova-ensemble,
author="Glazkova, Anna
and Glazkov, Maksim
and Trifonov, Timofey",
editor="Chakraborty, Tanmoy
and Shu, Kai
and Bernard, H. Russell
and Liu, Huan
and Akhtar, Md Shad",
title="g2tmn at Constraint@AAAI2021: Exploiting CT-BERT and Ensembling Learning for COVID-19 Fake News Detection",
booktitle="Combating Online Hostile Posts in Regional Languages during Emergency Situation",
year="2021",
publisher="Springer International Publishing",
address="Cham",
pages="116--127",
isbn="978-3-030-73696-5"
}

@ARTICLE{Kumar-ensemble,
  author={Kumar, Abhinav and Singh, Jyoti Prakash and Singh, Amit Kumar},
  journal={IT Professional}, 
  title={COVID-19 Fake News Detection Using Ensemble-Based Deep Learning Model}, 
  year={2022},
  volume={24},
  number={2},
  pages={32-37},
  doi={10.1109/MITP.2022.3149140}}

@InProceedings{
    das2021CovidFakeNews,
    author="Das, Sourya Dipta
    and Basak, Ayan
    and Dutta, Saikat",
    editor="Chakraborty, Tanmoy
    and Shu, Kai
    and Bernard, H. Russell
    and Liu, Huan
    and Akhtar, Md Shad",
    title="A Heuristic-Driven Ensemble Framework for COVID-19 Fake News Detection",
    booktitle="Combating Online Hostile Posts in Regional Languages during Emergency Situation",
    year="2021",
    publisher="Springer International Publishing",
    address="Cham",
    pages="164--176",
    isbn="978-3-030-73696-5"
}
